HelloWorld! An Instructive Case for the Transformation Tool Contest

This case comprises several primitive tasks that can be solved straight away with most transformation tools. The aim is to cover the most important kinds of primitive operations on models, i.e. create, read, update and delete (CRUD). To this end, tasks such as a constant transformation, a model-to-text transformation, a very basic migration transformation or diverse simple queries or in-place operations on graphs have to be solved. The motivation for this case is that the results expectedly will be very instructive for beginners. Also, it is really hard to compare transformation languages along complex cases, because the complexity of the respective case might hide the basic language concepts and constructs.

==> eptcsdata.tex <==
\providecommand{\firstpage}{22}
\providecommand{\publicationstatus}{Van Gorp, Mazanek and Rose (Eds.): \\Fifth Transformation Tool Contest (TTC 2011)\\
EPTCS 74, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.74.4}{10.4204/EPTCS.74.4}}
\pdfoutput=1

